MathNet: Haar-Like Wavelet Multiresolution-Analysis for Graph Representation and Learning

Graph Neural Networks (GNNs) have recently caught great attention and achieved significant progress in graph-level applications. In this paper, we propose a framework for graph neural networks with multiresolution Haar-like wavelets, or MathNet, with interrelated convolution and pooling strategies. The underlying method takes graphs in different structures as input and assembles consistent graph representations for readout layers, which then accomplishes label prediction. To achieve this, the multiresolution graph representations are first constructed and fed into graph convolutional layers for processing. The hierarchical graph pooling layers are then involved to downsample graph resolution while simultaneously remove redundancy within graph signals. The whole workflow could be formed with a multi-level graph analysis, which not only helps embed the intrinsic topological information of each graph into the GNN, but also supports fast computation of forward and adjoint graph transforms. We show by extensive experiments that the proposed framework obtains notable accuracy gains on graph classification and regression tasks with performance stability. The proposed MathNet outperforms various existing GNN models, especially on big data sets.

==> cache/IEEEversion/c_Preliminary.tex <==
\section{Technical Supports}
\label{preliminary}
We define a set of input to be studied as $\Gamma = \{(\mathcal{G}_1, X_1), (\mathcal{G}_2, X_2), ..., (\mathcal{G}_M, X_M)\}$ with graph $\mathcal{G}_g$ and features $X_g$ on it. A graph-level task aims at learning the hidden representation for each graph $(\mathcal{G}_g, X_g)$ to predict its label $\mathcal{Y}_g$ in labels $\{\mathcal{Y}_1, \mathcal{Y}_2, ..., \mathcal{Y}_M\}$. For an undirected and weighted graph instance $\mathcal{G}_g = (\mathcal{V}_g, \mathcal{E}_g, \mathcal{W}_g)$, the $\mathcal{V}_g = \{v_{1}, v_{2}, ..., v_{N_g}\}$ is a non-empty finite set of $|\mathcal{V}_g| = N_g$ vertices, and $\mathcal{E}_g \subset \mathcal{V}_g \times \mathcal{V}_g$ is a set of edges that can be represented as a weighted adjacency matrix $\mathcal{W}_g \in \mathbb{R}^{N_g \times N_g}$. %\textcolor{orange}{[Bingxin: Should we explain (J) here, if we are going to use it?]\WangC{We do not need to mention $J$ here yet. It has not been related to the chain yet. Also, $N$ is used to represent the number of nodes of $\mathcal{G}$; we can use $M$ to denote the number of data samples.} }


\subsection{Spectral Graph Convolution}
The spectral method defines graph convolution by an orthogonal basis on the graph.
% As an alternative way of embedding structural data into a manifold, graph signal processing defines the convolution in the spectral domain and constructs wavelet-like data representation \cite{bronstein2017geometric}. 
For an arbitrary graph, a spectral convolution transforms the input signal $X^{\text{in}}$ through the network trainable filter $G$
\begin{align}
 \widetilde{X}^{\text{in}} &= X^{\text{in}}W;\notag\\
    X^{\text{out}} &= \sigma(\Phi G \Phi^{-1} \widetilde{X}^{\text{in}}).\label{spectralConv}
\end{align}
%\MingC{Pay attention that the feature dimension of $X^{\text{in}}$ here should be one. Otherwise, the matrix formulation is not correct.}
where $\sigma(\cdot)$ is the non-linear activation function and $\Phi$ is the spectral basis matrix associated with the weighted adjacency matrix $\mathcal{W}$. The weight matrix $W\in \mathbb{R}^{d^{\rm in}\times d^{\rm out}}$ provides an affine transform of the input $X^{\rm in}\in \mathbb{R}^{N\times d^{\rm in}}$ to $\widetilde{X}^{\rm in}\in \mathbb{R}^{N\times d^{\rm out}}$. A spectral convolution can be defined by (discrete) adjoint and forward spectral transforms: the adjoint spectral transform $\Phi^{-1}$ maps $\widetilde{X}^{\rm in}$ from the vertex domain to the spectral domain; the filter $G$ processes feature information by the Hadamard product with the transformed graph data; the forward spectral transform $\Phi$ transmits the information back to the vertex domain to accomplish the convolution. Here, we have used a weight detaching trick in \Eqref{spectralConv}, i.e., conducting feature transformation $X^{\text{in}}W$ before performing the graph convolution, to reduce the parameter complexity from $O(N\times d^{\rm in}\times d^{\rm out})$ to 
$O(N+d^{\rm in}\times d^{\rm out})$.

People have proposed many ways to generate spectral-based convolution. For example, graph Fourier transforms \cite{shuman2013emerging} define the transform matrix $\Phi$ by the graph Laplacian. Graph wavelet neural networks \cite{xu2018graph} use the graph wavelet transforms, which provides a sparse and localised convolution for GNN.

The network filter $G$ plays a similar role as an image denoising task, where one uses low-pass filters to eliminate the noise in high frequencies. In GNNs, the network filter structure is data-driven and learned from the input graph data. The adaptivity to the data determines which part of the signals should be preserved, passed, or filtered out.


\subsection{Coarse-grained Chain Encoder}
\begin{figure}
  \centering
  \includegraphics[width=.45\textwidth]{vecFig/fig1.pdf}
  \caption{The hierarchical relationship of graph data $\Gamma$, an individual graph $\mathcal{G}$ and its coarse-grained graph $\mathcal{G}^{(j)}$ with $j = 0, 1, 2$ as a snapshot of coarse-grained chain. The level-wise Haar bases for every graph instance are generated from the constructed chain, and they are acting as the guidance of the corresponding graph convolution and graph pooling operations.}
  \label{fig1}
\end{figure}
Our graph convolution and graph pooling are based on a \emph{coarse-grained chain} of the graph. We employ graph coarsening to construct the chain. The target of coarsening is to partition a graph $\mathcal{G}$ into smaller meaningful clusters. By recursively downsampling vertices and creating new adjacent matrices, a hierarchical architecture is created to fold similar local features together. The clustering contributes to a chain of graphs. Each member at the layer coarser than the finest layer is a \emph{coarse-grained graph} of its finer layer. The graph nodes from a coarser layer are called parents, and the nodes from a finer layer are called children.

To be precise, a coarse-grained chain is a sequence of graph
\begin{equation*}
\mathcal{G}^{J \rightarrow J_0} \coloneqq 
(\mathcal{G}^{(J)}, \mathcal{G}^{(J-1)}, ..., \mathcal{G}^{(J_0)}),
\end{equation*} 
where $J > J_0$. In particular, we call $\mathcal{G}^{(J)}$ \textit{the finest level} or \textit{the bottom level} and it is inherited from the original graph. We recognise $\mathcal{G}^{(J_0)}$ as \textit{the coarsest level} or \textit{the top level}. The vertices at level $j$ is denoted by
\begin{equation*}
\mathcal{V}^{(j)} = \{v_{1}^{(j)}, ..., v_{N^{(j)}}^{(j)}\},
\end{equation*}
where $N^{(j)} \coloneqq |\mathcal{V}^{(j)}|$ indicates the number of vertices in graph $\mathcal{G}^{(j)}$. The complete chain structure can be constructed via either spectral or non-spectral clustering algorithms. Given the finest graph $\mathcal{G}^{(J)}$, we group $N^{(J)}$ vertices into $N^{(J-1)}$ clusters. Each cluster is a new vertex at the coarser level $\mathcal{G}^{(J-1)}$. The remaining coarser levels could be found accordingly until we reach the coarsest level $\mathcal{G}^{(J_0)}$. For any level $j$ coarser than the finest, the $k$th vertex also represents the $k$th cluster of $\mathcal{G}^{(j+1)}$ and some cluster for any finer levels. 
Each $v_i^{(j+1)}$ at level $j+1$ from the $k$th cluster is called a \textit{child} of the cluster, and $v_{k}^{(j)}$ at level $j$ is the \textit{parent} of all the elements in the same set. 

There are many clustering methods, such as $k$-means\cite{lloyd1982least}, METIS \cite{karypis1995metis} and spectral clustering \cite{von2007tutorial}. By the time complexity, the METIS is faster than spectral clustering, which is faster than $k$-means. In terms of the clustering accuracy, spectral clustering and $k$-means are better than METIS. In practice, we will consider the trade-off between the computational cost and clustering precision.

\subsection{Haar Orthonormal System and Local Filtration}
Applying the conventional graph Fourier transform to GNNs is straight-forward and a conceptually important breakthrough. However, it comes with significant computational deficiency and lacks scalability. One way to overcome the computational intractability is to replace the Fourier basis by another orthonormal basis on the graph. The underlying orthonormal system should be feasible to compute while allowing efficient algorithms for spectral transforms. One such candidate is the Haar orthonormal basis introduced by \cite{gavish2012sampling,chui2015representation,wang2019tight}.

Haar basis is a sparse orthogonal system that adapts to a coarse-grained chain of the underlying graph. To construct the graph Haar basis, we form a hierarchical structure $\mathcal{G}^{J \rightarrow J_0}$ through progressively `folding' the vertices of a graph. The local orthogonal system is then dilated along the chain until obtaining the global system at the bottom level, see Section~\ref{methodology} for more details. 

The Haar orthonormal system is completely constructive via a filtration (i.e. the chain). For the graph at each level of the coarse-grained chain, we establish an orthonormal basis. The basis at the finest layer becomes the global Haar basis of the underlying graph. 

The Haar basis guarantees the orthogonality and locality of the system. 
The top-down procedure of basis generation creates a sparse yet non-redundant set of system, and the clustering of the chain connects the bases on two neighbouring layers of the chain. It with the locality sparsifies the Haar basis matrix and supports the feasibility of fast computation on scalable data.
With such construction, the Haar system acquires the ability to handle graph input with changing size and structure. It naturally enables processing of different graphs with an embedded pooling operation, as we introduce below.

==> cache/IEEEversion/d_Methodology.tex <==
\section{The Proposed HaarNet}
\label{methodology}
We present our proposed model in this section. We focus on the model that works for graph classification and regression tasks. It includes three key operation blocks: orthogonal system construction,  Haar graph convolution and hierarchical Haar graph pooling.

We first have a glance at the network architecture of our HaarNet model for graph classification and regression tasks, as illustrated in Fig.~\ref{fig3}. As a typical GNN model, it contains Haar graph convolution, Haar graph pooling and fully connected layers in turn. Both the Haar graph convolution and pooling operations are defined by Haar Global Orthonormal Basis (HGOB) on an individual input graph $\mathcal{G}$. HGOB is fully constructive and based on a chain of the graph $\mathcal{G}$. The Haar graph convolution exploits the fast Haar transforms to extract the graph data in the Haar wavelet domain. The Haar graph pooling utilises the \emph{compressive Haar transforms} filter out the high pass but keeps the low pass in the multi-resolution decomposition of the Haar wavelet system on the graph. In consequence of the tree structure of the Haar system, the graph size after the Haar pooling becomes identical, which enables the HaarNet to cope with graph samples with varying size and structure. We now introduce the computational principle for each unit of operation.

\subsection{Global Orthonormal Basis}
\label{methodology_haarBasis}
\begin{figure}
  \centering
  \includegraphics[width=.45\textwidth]{vecFig/fig2.pdf}
  \caption{A toy example of fast Haar basis construction. For a given graph $\mathcal{G}$, a bottom-up coarse-grained chain structure is first generated by clustering. The Haar global orthogonal basis is then constructed following a top-down fashion. Each parent basis at level $j$ is dilated to level $j+1$. The number of dilated bases is determined by the number of its children at level $j+1$. The generated Haar basis is sparse and properly sorted. See Section~\ref{methodology_haarBasis} for more details.}
  \label{fig2}
\end{figure}
For the graph $\mathcal{G}^{(j)}$ of a chain at the $j$th layer, the constructed \emph{Haar basis} is a set of $N^{(j)}$ vectors of length $N^{(j)}$. It forms a square matrix $\Phi^{(j)}$ of size $N^{(j)}$.
By its nature, the Haar basis at each layer can be decomposed into `low-pass' and `high-pass':
\begin{equation*}
    \Phi^{(j)} = \left[\Phi_{\rm low}^{(j)}\;\; \Phi_{\rm high}^{(j)}\right].
\end{equation*}
Here $\Phi_{\rm high}^{(j)}$ can be generalised to multiple high passes.
At the finest layer $\mathcal{G}^{(J)}$, we call $\Phi^{(J)}$ the \emph{Haar global orthonormal basis} for the original graph $\mathcal{G}$, or simply \emph{global Haar basis} for $\mathcal{G}$.
The global Haar basis provides a multi-resolution decomposition and reconstruction, which is useful for sparsifying the pair-wise constant interaction in the input signal and reserving the mutual information between local and global embeddings \cite{ye2018deep}. 

The global Haar orthogonal basis has been studied extensively in \cite{gavish2012sampling,chui2015representation,wang2019haarpooling,wang2019tight}. In particular, \cite{chui2015representation,wang2019haarpooling,wang2019tight} show explicit construction and fast implementation for the Haar system. We aim at obtaining a sequence of the Haar orthogonal bases (matrices)
\begin{equation*}
    \bigl\{\Phi^{(J_0)}, \Phi^{(J_0+1)}, \dots, \Phi^{(J)}\bigr\},
\end{equation*}
where $\Phi^{(j)}$ is the basis matrix corresponding to the graph $\mathcal{G}^{(j)} = (\mathcal{V}^{(j)}, \mathcal{E}^{(j)}, \mathcal{W}^{(j)})$ at the $j$th level of the chain, which contains is composed of $N^{(j)}$ basis vectors
\begin{equation*}
    \Phi^{(j)} = \bigl(\phi_1^{(j)}, \phi_2^{(j)}, ..., \phi_{N^{(j)}}^{(j)}\bigr).
\end{equation*}

The construction of the Haar system follows a top-down manner to recursively adopt the \textit{characteristic function} and the \textit{extension function} along the coarse-grained chain $\mathcal{G}^{J \rightarrow J_0} = (\mathcal{G}^{(J)}, \mathcal{G}^{(J-1)}, ..., \mathcal{G}^{(J_0)})$. 
We start from preparing the node set $\mathcal{V}^{(j-1)} = \{v_{1}^{(j-1)}, ..., v_{N^{(j)}}^{(j-1)}\}$ (which is ordered here for illustration simplicity) for the coarser level by sequencing the supernodes via their degrees or weights.


\subsubsection{Characteristic Function}
We define a characteristic function $\chi_{k}^{(j)}$ for the $k$th cluster in $\mathcal{V}^{(j)}$. It is also associated with the $k$th vertex $v_{k}^{(j-1)}$ in $\mathcal{V}^{(j-1)}$. 
\begin{equation}
    \chi_{k}^{(j)}:=\left\{
\begin{array}{ll}
1, & v_i^{(c)}=v_{k}^{(j-1)}, \\
0, & \text{otherwise}. 
\end{array}\right.
\end{equation}
We use $\chi_{k}^{(j)} = 1$ to determine whether the vertex $v_i^{(j)}$ belongs to the $k$th cluster. The condition is equivalent to have a parent $v_{k}^{(j-1)}$ at the coarser $(j-1)$th level.


\subsubsection{Extension Function}
The dimension of each Haar Basis is determined by the number of vertices at that level. Constructing $\Phi^{(j)}$ from $\Phi^{(j-1)}$ requires the size of the orthogonal system to be extended from $N^{(j-1)} \times N^{(j-1)}$ to $N^{(j)} \times N^{(j)}$. We achieve the target in the following two steps.
We start from extending the column vectors $\{\phi_{1}^{(j-1)}, ..., \phi_{N^{(j-1)}}^{(j-1)}\}$ vertically to obtain $N^{(j-1)}$ vectors of length $N^{(j)}$. The $l$th new basis, denoted by $\phi_{l}^{(j)*}$, is extended from
\begin{equation}
\phi_{l}^{(j)*} \coloneqq \frac{\phi_{l}^{(j-1)}}{\sqrt{\xi_{l}^{(j)}}},
\label{haarBasisExtend1}
\end{equation}
where $\xi_{l}^{(j)}$ is the size of the $l$th cluster at level $j$. The vertices within the cluster share the same parent of $v_{l}^{(j-1)} \in \mathcal{V}^{(j-1)}$ at the coarser level $j-1$.

Next we apply the Gram-Schmidt process and extend the number of orthogonal basis to match the number of vertices at level $j$. Each $\phi_{l}^{(j)*}$ from \Eqref{haarBasisExtend1} would be split into $\xi_{l}^{(j)}$ basis. For $k = 2, 3, ..., \xi_{l}^{(j)}$, we define
\begin{equation}
\phi_{l,k}^{(j)} \coloneqq \sqrt{\frac{\xi_{l}^{(j)}-k+1}{\xi_{l}^{(j)}-k+2}}\left(\chi_{k-1}^{(j)}-\frac{\sum_{i=k}^{\xi_{l}^{(j)}} \chi_{l,i}^{(j)}}{\xi_{l}^{(j)}-k+1}\right).
\label{haarBasisExtend2}
\end{equation}
Accumulating all $\phi_{l,k}^{(j)}$ together for all the $l$ clusters, and we obtain an orthonormal basis for $\ell_2(\mathcal{G}^{(j)})$ at the $j$th layer from the $(j-1)$th layer. The vectors of the basis gives the basis matrix $\Phi^{(j)} \in \mathbb{R}^{N^{(j)} \times N^{(j)}}$, which we call it a Haar transform on $\ell_2(\mathcal{G}^{(j)})$. For any chain structure $\mathcal{G}^{J \rightarrow J_0}$, we can always apply the `vertical extending - horizontal extending' scheme and find the Haar orthogonal basis for the next finer level. When $j = J$, we reach the finest level and the corresponding $\Phi^{(J)}$ is called the \textit{Haar Global Orthonormal Basis}, or HGOB, for the original graph $\mathcal{G}$.

One special case is the coarsest level $J_0$, where each vertex belongs to an exclusive cluster, and there is no further coarser level `$J_{-1}$'. We modify \Eqref{haarBasisExtend1} and \Eqref{haarBasisExtend2} accordingly by defining $\phi_{l}^{(j-1)} = 1$ and $\xi_{l}^{(J_0)} = N^{(J_0)}$. For $l = 2, 3, ..., N^{(J_0)}$, we have
\begin{equation}
\begin{aligned}
\phi_{1}^{(J_0)} &\coloneqq \frac{1}{\sqrt{N^{(J_0)}}}\\[1mm]
\phi_{l}^{(J_0)} &\coloneqq \sqrt{\frac{N^{(J_0)}-l+1}{N^{(J_0)}-l+2}}\left(\chi_{l-1}^{(J_0)}-\frac{\sum_{i=l}^{N^{(J_0)}} \chi_{i}^{(J_0)}}{N^{(J_0)}-l+1}\right). \notag
\end{aligned}
\end{equation}
We now utilise the constructed bases $\{\phi_l^{(j)}\}_{l=1}^{N^{(j)}}$, $j=J_0, \dots, J$ on the chain to define a graph convolution and graph pooling, see Sections~\ref{sec:convlayer} and \ref{sec:poollayer}.


\subsection{Convolutional Layer}
\label{sec:convlayer}
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{vecFig/fig3.pdf}
  \caption{An illustration of \textsc{HaarNet} structure with 2 Haar blocks and a fully connected layer. We unify a block of the \textsc{HaarNet} structure to cover Haar graph convolutional layer(s) following Haar graph pooling layer(s) (red rounded-rectangles). Given a set of graph $\Gamma$, we first construct the Haar basis sets $\Phi^{(2)}$ and $\Phi^{(1)}$ along the coarse-grained chain for each graph $\mathcal{G}_i$ at level $j = 2$ and $1$. The constructed orthonormal systems are applied to support convolutional and pooling operations. The formulations inside one Haar block only involves one basis set. For the first Haar block, we take the ordered HGOBs $\Phi^{(2)} = \{\Phi_1^{(2)}, \Phi_2^{(2)}, ..., \Phi_M^{(2)}\}$ to guide the adjoint and forward Haar transforms. The process, as detailed in the blue rounded-rectangle, constitutes one Haar graph convolutional layer. The filter matrix $G$ is shared among graphs at the same level, and it is universally applicable on different graphs after the padding strategy on the Haar basis of $\Phi$. For the sake of conciseness, we only demonstrate one convolutional layer. However, in practice, it could be repeated multiple times. We send the final output of the convolutional layer (after activation) to the pooling layer, where we utilise the compressive Haar transforms to filter out the high-pass signals and reserve low-pass signals. The coarsening process is implemented by the transform of $\Phi^{(2)}$; the $\Phi^{(1)}$ (yellow rounded-rectangles) gives the size of the output of the downsampling procedure. Note that the network component is not constrained to the illustration, and a specific application should determine the employed structure. For clarity, we also exclude some common technical details like activation and weight detaching in this visualization.}
  \label{fig3}
\end{figure*}
This section presents the motivation and details of the core operations in a Haar Convolutional Layer. We include the forward and adjoint Haar transforms for the Haar global orthonormal basis on the graph as constructed above, and their fast implementations as inspired by \cite{li2019haar}. Also, we propose a padding strategy for training the global structure of filtration.

In this paper, instead of applying the Fourier basis, we use the Haar basis for the $U$ in the graph convolution in \Eqref{spectralConv}. We rule out the Fourier basis of the graph Laplacian to avoid the fussy computation of a dense matrix. The computation cost of eigendecomposition and discrete Fourier transform increase dramatically with the graph size, which in no circumstance is desirable. In contrast, our Haar basis is constructed from the coarse-grained chain with clustering properties. The compressive workflow provides a sparsified operator $\Phi$ to support the fast computation of the adjoint and forward Haar transforms. We adopt the notation from the previous sections and detail the fast implementation below.
% The compressive information is accumulated along the hierarchical chain. 

\subsubsection{Adjoint Haar Transform}
On level $j$ of $\mathcal{G}_i^{(j)}$, the adjoint Haar transform formulates a set of \textit{Haar coefficients} for $X^{\text{in}}$
$$
(\Phi^{(j)})^{T} X^{\text{in}} = \bigl(c_{1}^{(j)}, ..., c_{N^{(j)}}^{(j)}\bigr) \in \mathbb{R}^{N^{(j)} \times d}.
$$
The $l$th coefficient with respect to $v_{l}^{(j)}$ is accumulated from its children vectors $v_{l'}^{(j)}$ at level $j+1$
\begin{align}
c_{l}^{(j)} &\coloneqq 
\sum_{v_{l}^{(j)} \in \mathcal{V}^{(j)}} \omega_{l}^{(j)} S_{l}^{(j)} \phi_{l}^{(j)*} \label{adft}\\
\omega_{l}^{(j)} &\coloneqq \frac{1}{\sqrt{\xi_{l}^{(j)}}} \label{weight}\\
\mathcal{S}_{l}^{(j)} &\coloneqq \sum_{v_{l'}^{(j+1)} \in v_{l}^{(j)}} \omega_{l'}^{(j+1)} \mathcal{S}_{v_{l'}}^{(j+1)}. \label{weightedSum}
\end{align}
In a nutshell, the coefficient $c_{l}^{(j)}$ for $v_{l}^{(j)}$ reflects the weighted sum of information from its children. The \textit{weight factors} for each child is defined by \Eqref{weight}, and the recursive summation follows \Eqref{weightedSum}.


\subsubsection{Forward Haar Transform}
The forward Haar transform sends the Haar coefficients back to the vertex domain. Given a set of coefficients $c = \{c_{1}, ..., c_{N}\}$ at the finest level $\mathcal{G}^{(J)}$, the reconstruction is, for $l = 1, ..., N,$
\begin{align}
\Phi c_{l} &\coloneqq \sum_{j=J_0}^{J} W_{l}^{(j)}\left(
\sum_{k = N^{(j-1)}+1}^{N^{(j)}} c_{k} \phi_{k_j}^{(j)*}
\right)\\
W_{l}^{(j)} &\coloneqq \prod_{k=J_0}^{j} \frac{1}{\omega_{k}^{(j)}} \quad \text { for } j=J_{0}, \ldots, J-1.
\end{align}
For a vertex $v_{k}^{(J)}$, we accumulate weighted information from its parents $v_{k_j}^{(j)}$ at each coarser level $j$ for $j = J_0, ..., J-1$. The weight factor $\omega_{k}^{(j)}$ follows the same format as in \Eqref{weight}.


\subsubsection{Padding Strategy}
The trainable filter matrix $G$ is learned in the wavelet domain and it is used to process the Haar coefficients. Conventionally, the matrix for an individual graph $\mathcal{G}^{(j)}$ is constructed as a diagonal matrix of size $N^{(j)}$. In graph-level tasks, different graphs share the same number of features, but contain varying number of nodes. To eliminate the inconsistency and apply an identical filtration rule along the full graph data set, we consider a padding strategy on Haar bases and extend all bases to a unified length. The modified basis matrix then has the form $\Phi^{(j)} \in \mathbb{R}^{N^{(j)} \times N_{\text{max}}^{(j)}}$, $N_{\text{max}}^{(j)} \coloneqq \max\{N_1^{(j)}, ..., N_M^{(j)}\}$, where we fill the extra columns by $\mathbf{0}$ vectors.


\subsection{Pooling Layer}
\label{sec:poollayer}
The well-constructed Haar Orthogonal System is applied to perform the pooling operation along the prepared coarse-grained chain. We summarize the motivation and key calculations. For more details we refer the readers to the technical analysis and proofs in \cite{wang2019haarpooling}. For an input graph $\mathcal{G}$ and its chain $\mathcal{G}^{J\to J_0}$, the \emph{Haar pooling} consists of $J-J_0$ Haar pooling layers in the GNN. The Haar pooling of the $j$th layer is given by
\begin{equation}
\widehat{X}^{(j)} = (\widetilde{\Phi}^{(j)})^T X^{(j)} 
\end{equation}
for $j= J-1,J-2,\dots,J_0$, where $X^{(j)} \in \mathbb{R}^{N_{\rm max}^{(j)} \times d}$ is constituted from the output of the last convolutional layer. The pooling operator $\widetilde{\Phi}^{(j)}$ takes the first $N^{(j-1)}$ columns from the associated Haar Basis $\Phi^{(j)}$ at the level $j$ of the chain. As a result, the output of this Haar Pooling layer downsamples the matrix size to $\mathbb{R}^{N^{(j-1)} \times d}$ for each graph. At the last Haar pooling layer, the output has a standard size $\mathbb{R}^{1\times d'}$ for each graph. The output feature dimension $d'$ is determined by the external weights of graph convolutional layers.

The compressive Haar transform follows a similar fast computational strategy as the adjoint transform in the convolutional layer. To minimise the number of summation and products operations, we modify the weighted sum of signal information in \Eqref{weightedSum} by pre-gathering the feature vectors from child nodes to the coarsest possible level. Formally, for the input feature $X^{(j)} \in \mathbb{R}^{N_{\rm max}^{(j)}\times d}$ at the $j$th layer, we prepare the weighted sum by
\begin{align}
S^{(j)} &\coloneqq X^{(j)} \label{parent} \\
\mathcal{S}_{l}^{(i)} &\coloneqq \sum_{v_{l'}^{(i+1)} \in v_{l}^{(i)}} \omega_{l'}^{(i+1)} \mathcal{S}_{v_{l'}}^{(i+1)}. \label{children}
\end{align}
We define $i \leq j$ to represent the coarsest possible layer where the corresponding $\phi_{\ell}^{(i)}$ is the $\ell$th member of the orthonormal basis $\{\phi_{\ell}^{(i)}\}_{\ell=1}^{N^{(i)}}$. At each level $j$, the compressive Haar transform inherits full information from the first $N^{(j-1)}$ feature vectors which are elected as parent nodes at level $j-1$. The rest $N^{(j)} - N^{(j-1)}$ child nodes contribute their feature information to the coarsest possible layer. The information from parents and children are gathered via \Eqref{parent} and \Eqref{children}, respectively. The calculation of weights $\omega_{l'}^{(i+1)}$ follows \Eqref{weight}, and the final result of the compressive Haar transform is then given by \Eqref{adft}.

The pooling operation is essential to our graph regression and classification tasks. It unifies graph embedding for a given set of graphs with different structure and sizes. Such unanimity allows our model to handle graph data without further pre-processing. Besides, adopting Haar Pooling layers benefits our GNN from three particular perspectives. First, it takes only the low-frequency coefficients to approximate the original data. The noise in high-frequency coefficients are stripped out, and the remaining information is adequately purified. As a result of performing local graph Fourier transformation, the subgraph structure and the node features are utilised for generating the supernode representations. As pointed out by \cite{Morris2017Glocalized,zhang2018end}, the compound information maximises the model performance. Also, \cite{wang2019haarpooling,ye2018deep} have shown that the Haar basis is closely related to the average pooling operation, which incorporates the spatial behaviour of the graph signal. Such pooling strategy has attested its power in many practical applications of CNN and GNN.

==> cache/Introduction_old.tex <==
\section{Introduction}
%\MingC{The first para. is too long. just say a general background around GNNs. It is better to move the last sentence to Paragraph 2?}
The practical importance of learning with graph-structured data has been well-explored in many previous study \cite{bronstein2017geometric,zhou2018graph,wu2020comprehensive,vijay2020benchmarking}. %jin2018learning,zhang2018end,ying2018graph,xu2019spatial,
%\MingC{Yes, add more refs. here. Also, we only need survey papers here, rather than technical ones}
Depending on the structure of input data, the learning task includes representation learning in node-level \cite{kipf2016semi,veli2018graph,hoang2019revisiting} and graph-level \cite{xu2018powerful,ying2018hierarchical,ma2019graph,wang2019haarpooling}, such as node/graph classification and regression. This paper focuses on graph classification tasks. As a generalised version of image classification, graph classification aims at forecasting the label of a new graph with adjacency structure. Motivated by the traditional Convolutional Neural Network (CNN) models, the Graph Neural Network (GNN) structures usually involve \textit{convolutional layers} and \textit{pooling layers} to transform, propagate, aggregate and extract node features by exploiting the structural information of the input graph \cite{wu2020comprehensive}. 

% convolutional layer
By choice of the domain where an operation is defined, researchers have proposed the spectral method and spatial method for graph convolution. % and graph pooling.}
% Graph convolutional layers embed node features from a given graph. Two types of \textit{graph convolution methods} have been developed so far with the spatial and the spectral graph convolution methods. 
% spatial
%\MingC{This para. also needs improvements. Pay attention to the logicality. Start by saying "There are generally two schemes for constructing graph convolution: spectral and spatial methods.“ In particular, remember to mention the messgae passing for spatial method. Remember to cite the bridging spatial/spectral domain papers, etc.}
The spatial method defines the graph convolution on a localized patch of the node in vertex space \cite{micheli2009neural,atwood2016diffusion,yan2018spatial,bhattacharya2019step}. Such method usually follows the format of message passing, where node information is transit along the edges and paths and the representation of a central node is built recursively upon its neighbourhoods \cite{gilmer2017neural}. During the aggregation process, the attention mechanism was proposed to assign the weights implicitly in the network structure \cite{veli2018graph,xu2018how}. 
% spectral
On the other hand, the spectral graph method proposes to carry out the convolution operation in a frequency domain, such as the Fourier domain and the wavelet domain. It utilises the Fourier/wavelet discrete convolution to design a node embedding for graph \cite{bruna2013spectral}. The feature information on each node is passed from the vertex domain to the frequency domain through the spectral basis representation of the graph data. The Fourier/wavelet coefficients are then involved to perform the convolution operation \cite{henaff2015deep}. 
Conventional Fourier methods use graph Laplacian and its eigenpairs, which however suffer from the high computational cost of eigendecomposition. Modifications on the filter are proposed to find its close approximation and avoid the eigendecomposition or the exploding amount of filter coefficients \cite{defferrard2016convolutional,kipf2016semi}. Alternatively, the wavelet method replaces the graph Fourier transform to find a sparse representation for the basis system \cite{xu2018graph,li2019haar}. It shall be emphasized that many spatial and spectral methods are compatible approaches that processing graph information from different angels \cite{chen2020bridging,balcilar2020bridging}. 

% pooling layer
Graph pooling layers are generally \Wang{used in graph-level learning problems, which unifies} the vector embedding of each graph input. 
Different from the predominant graph kernel methods \cite{kondor2016multiscale,zhang2018end,kriege2020survey}, graph pooling methods generate graph embedding from subgraphs or supernodes. The concatenation maximizes graph \Wang{expressivity} power \Wang{by learning} the feature information without sacrificing the computational speed or structural flexibility, which are long-existent problems on graph kernel methods \cite{wu2020comprehensive}. In \cite{duvenaud2015convolutional,atwood2016diffusion,gilmer2017neural}, people consider global pooling methods to capture feature information with a dense layer. 
While the \Wang{neighbourhood structure expression} plays a pivotal role in \Wang{graph learning, the} hierarchical pooling strategy \cite{ying2018hierarchical,gao2019graph,cangea2018towards,knyazev2019understanding} is introduced to aggregate the feature information into a super-node. The cascading workflow maintains \Wang{the} maximum feature information but loses the completeness of graph topological information. Moreover, the `black-box' downsampling process is fully data-driven but lacking interpretability. The practical explanation is implicit for the scoring matrix. 
Alternatively, \cite{noutahi2019towards,ma2019graph} take \Wang{the graph} Laplacian into account to combine feature information and geometric information. Such spectral-based techniques drop the detailed information layer by layer to extract smoothing feature representations. Unfortunately, both methods \Wang{have high computational cost mainly due to} eigendecomposition, which becomes \Wang{the most significant} barrier for them to go viral. 

\Wang{The application of the wavelet transform in neural networks has attracted increasing attention recently, where the multiscale structure of the graph wavelet representation proves an effectiveness and efficiency scheme in various tasks including de-noising and feature extraction \cite{williams2016advanced,oord2016wavenet,liu2019multi}.}
\Wang{Recently, a new pooling strategy was proposed by \cite{wang2019haarpooling} as the compressive Haar transforms of the input node feature and achieves the state of art performance on graph classification/regression tasks.} %\MingC{This sentence 'Recently......' is too long. }
% It inherits the conventional graph convolutions network (GCN) \cite{kipf2016semi} for the convolutional layers to make the best of neighbouring information. 
% While engaging local graph properties could benefit node-level tasks, appending global features is suggested more powerful for graph-level applications \cite{Morris2017Glocalized,zhang2018end}. 
\Wang{In this paper, we propose a GNN which convolution and pooling both defined in terms of the same graph Haar basis. As compared to existing GNNs, this strategy is distinct in the following three aspects.}
\begin{itemize} 
    \item \textbf{\Wang{Efficient graph} convolution and pooling with hierarchical architecture}: We generate coarse-grained tree structure for graphs to support fast computation on \Wang{multiscale graph signal decomposition, and a} cascading pooling workflow. The constructed orthogonal bases guarantee sufficient sparsity to capture mutual information between local and global embeddings \Wang{with low computational cost}. Our method is not only capable of solving large-scale node-level \Wang{learning} problems, but also outstanding in handling graph-level problems.
    \item \textbf{Interpretable pooling strategy}\MingC{what does this mean? I think it is difficult to obtain interpretability/explainability.}\WangC{I think it is OK to say so, as the math expression of pooling is precise and simple; and the distinguishing of noise can be explained by low pass and high passes of Haar basis representation.}: Thanks to the fast spectral-based pooling strategy, our model separates the irregular patterns within a graph, which are essentially noise and redundancy that hurt the model performance. Compared to the \Wang{existing pooling} strategies, our feature selection is not only driven by data but also supported by solid theory from the perspective of signal processing. 
    \item \textbf{End-to-end network structure}: To the best of our knowledge, our method attempts for the first time to incorporate spectral-based convolutional and pooling layers in one GNN for graph \Wang{classification/regression task}. The pattern embedded in graph data is maximized from different angles. \Wang{By Haar basis, both local and global information is properly represented, and the topological and feature information of the graph data is then effectively extracted}. Aside from theoretically appealing, the superiority of \Wang{our Haar-based GNN} is also supported by empirical evidence.
    \item \MingC{One more point: Develop a unified framework for how to build graph neural networks with both spectral-based convolutional layers and pooling layers. Some existing GNNs indeed do not have a `unified' convolutional layer and pooling layer.}%\WangC{Agree, we can add this point as Ming mentioned.}
\end{itemize}

The rest of this paper is organized as follows. Section~\ref{preliminary} introduces the fundamental ideas that construct the spectral graph networks. Section~\ref{methodology} formulates the proposed Haar-based GNN method. In Section~\ref{experiment}, we test the proposed model on a variety of graph learning tasks, including classification tasks at both node and graph levels. Section~\ref{concusion} summarizes the paper together with discussion on related future work.


% cache----------------------------------
%First, the eigen-decomposition on graph Laplaacian could be tricky, which increases the difficulty of calculating the basis matrix for Fourier transform. Second, due to the lack of structural patterns, it is hard to formulate a fast computation for the adjoint transformation on the input signal. On top of that, the neglected spatial relationships in the spectral method prevents a smaller filter coefficients to be estimated.\\
%The spectral propagation rule embeds the localized information by allocating high weights for low-degree neighbors, and low weights for high-degree neighbors.


% turn to Haar wavelet transformation
% In addition to node features, the topological information is desired for graph downsampling. 
% instead of eigen-decomposition or Fourier transformaiton，我们借助wavelet transformation来实现fast computation。这种transformation的优点在


%CNN-WAV \cite{williams2016advanced} applies fast wavelet transform and creates versatile wavelet subbands to identify and store multi-resolutional characteristics. WaveNet \cite{oord2016wavenet} includes dilated-convolutions and extends the receptive field of the time window to capture sophisticated patterns with long-term memory. MWCNN \cite{liu2019multi} studies multi-level discrete wavelet transform with the U-net architecture. The multi-level structure improves model performance via a larger receptive field while controls the computational cost. Also, both filter dilation and average pooling are proved embedding within the modelling process. In addition to CNN, recent literature also start to such appealing architecture also draws increasing attention from GNN community \cite{williams2018wavelet,wang2019haarpooling}.


%We summarize the contribution in three-folds.
%\begin{itemize} 
%	\item %We argue the sufficiency of spatial graph network where the structure only consider k-hop neighborhoods for prediction. In order to develop a holistic view on the full dataset, the model is encouraged to derive the hybrid patterns both locally and globally so that similar incidents could better be defined and paired.
%	\item %The traditional spectral graph networks rely on Laplacian decomposition or Fourier transform. While theoretically appealing, the computational cost prevent the method from solving large-scale problems. To address the problem, we consider fast wavelet transformation with high sparsity. Not only the procedure promises an efficient algorithm implementation, but also it separate out the irregular patterns within the data, which is essentially noise that hurts the model accuracy.
%	\item %We introduce a new regularizer in the loss function to allow the network punishing the redundancy. By following the encoding – decoding process, the model is able to extract the most important filters while training the network without further pooling process. 
%\end{itemize}







==> cache/reference_old.tex <==
@inproceedings{wang2019tight,
  title={Tight framelets on graphs for multiscale data analysis},
  author={Wang, Yu Guang and Zhuang, Xiaosheng},
  booktitle={Wavelets and Sparsity XVIII},
  volume={11138},
  pages={111380B},
  year={2019},
  organization={International Society for Optics and Photonics}
}

@ARTICLE{bronstein2017geometric,
author={M. M. {Bronstein} and J. {Bruna} and Y. {LeCun} and A. {Szlam} and P. {Vandergheynst}},
  journal={IEEE Signal Processing Magazine},
 title={Geometric Deep Learning: Going beyond {Euclidean} data},
  year={2017},
  volume={34},
  number={4},
  pages={18-42},
  abstract={Geometric deep learning is an umbrella term for emerging techniques attempting to generalize (structured) deep neural models to non-Euclidean domains, such as graphs and manifolds. The purpose of this article is to overview different examples of geometric deep-learning problems and present available solutions, key difficulties, applications, and future research directions in this nascent field.},
  keywords={computational geometry;neural nets;geometric deep learning;Euclidean data;deep neural models;Convolution;Computational modeling;Euclidean distance;Machine learning;Convolutional codes;Social network services;Computer architecture},
  doi={10.1109/MSP.2017.2693418},
  ISSN={1558-0792},
  month={July}
}


@article{ye2018deep,
  title={Deep convolutional framelets: A general deep learning framework for inverse problems},
  author={Ye, Jong Chul and Han, Yoseob and Cha, Eunju},
  journal={SIAM Journal on Imaging Sciences},
  volume={11},
  number={2},
  pages={991--1048},
  year={2018},
  publisher={SIAM}
}

@article{shah2016construction,
  title={Construction of shift invariant M-band tight framelet packets},
  author={Shah, Firdous A},
  journal={TWMS Journal of Applied and Engineering Mathematics},
  volume={6},
  number={1},
  pages={102},
  year={2016},
  publisher={Elman Hasanoglu}
}

@article{daubechies2003framelets,
  title={Framelets: MRA-based constructions of wavelet frames},
  author={Daubechies, Ingrid and Han, Bin and Ron, Amos and Shen, Zuowei},
  journal={Applied and computational harmonic analysis},
  volume={14},
  number={1},
  pages={1--46},
  year={2003},
  publisher={Elsevier}
}

@article{han2013properties,
  title={Properties of discrete framelet transforms},
  author={Han, Bin},
  journal={Mathematical Modelling of Natural Phenomena},
  volume={8},
  number={1},
  pages={18--47},
  year={2013},
  publisher={EDP Sciences}
}

@article{kang2018deep,
  title={Deep convolutional framelet denosing for low-dose CT via wavelet residual network},
  author={Kang, Eunhee and Chang, Won and Yoo, Jaejun and Ye, Jong Chul},
  journal={IEEE transactions on medical imaging},
  volume={37},
  number={6},
  pages={1358--1369},
  year={2018},
  publisher={IEEE}
}

@article{skodras2007discrete,
  title={Discrete Wavelet Transform: An Introduction},
  author={Skodras, Athanassios},
  journal={HELLENIC OPEN UNIVERSITY JOURNAL OF INFORMATICS},
  volume={1},
  number={1},
  year={2007}
}

@article{abdelnour2004symmetric,
  title={Symmetric nearly shift-invariant tight frame wavelets},
  author={Abdelnour, A Farras and Selesnick, Ivan W},
  journal={IEEE Transactions on signal processing},
  volume={53},
  number={1},
  pages={231--239},
  year={2004},
  publisher={IEEE}
}

@inproceedings{
xu2018graph,
title={Graph Wavelet Neural Network},
author={Bingbing Xu and Huawei Shen and Qi Cao and Yunqi Qiu and Xueqi Cheng},
booktitle={ICLR},
year={2019},
url={https://openreview.net/forum?id=H1ewdiR5tQ},
}

@article{shuman2013emerging,
  title={The emerging field of signal processing on graphs: Extending high-dimensional data analysis to networks and other irregular domains},
  author={Shuman, David I and Narang, Sunil K and Frossard, Pascal and Ortega, Antonio and Vandergheynst, Pierre},
  journal={IEEE signal processing magazine},
  volume={30},
  number={3},
  pages={83--98},
  year={2013},
  publisher={IEEE}
}

@article{li2019haar,
  title={Haar Transforms for Graph Neural Networks},
  author={Li, Ming and Ma, Zheng and Wang, Yu Guang and Zhuang, Xiaosheng},
  journal={Neural Networks},
  year={2020, DOI: https://doi.org/10.1016/j.neunet.2020.04.028}
}

@article{zhang2018deep,
  title={Deep learning on graphs: A survey},
  author={Zhang, Ziwei and Cui, Peng and Zhu, Wenwu},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  year={2020, DOI: 10.1109/TKDE.2020.2981333}
}

@inproceedings{defferrard2016convolutional,
  title={Convolutional neural networks on graphs with fast localized spectral filtering},
  author={Defferrard, Micha{\"e}l and Bresson, Xavier and Vandergheynst, Pierre},
  booktitle={NeurIPS},
  pages={3844--3852},
  year={2016}
}

@article{kipf2016semi,
  title={Semi-supervised classification with graph convolutional networks},
  author={Kipf, Thomas N and Welling, Max},
  journal={arXiv preprint arXiv:1609.02907},
  year={2016}
}

@article{bruna2013spectral,
  title={Spectral networks and locally connected networks on graphs},
  author={Bruna, Joan and Zaremba, Wojciech and Szlam, Arthur and LeCun, Yann},
  journal={arXiv preprint arXiv:1312.6203},
  year={2013}
}

@inproceedings{
  jin2018learning,
  title={Learning Multimodal Graph-to-Graph Translation for Molecule Optimization},
  author={Wengong Jin and Kevin Yang and Regina Barzilay and Tommi Jaakkola},
  booktitle={International Conference on Learning Representations},
  year={2019},
  url={https://openreview.net/forum?id=B1xJAsA5F7},
}

@article{oord2016wavenet,
  title={Wavenet: A generative model for raw audio},
  author={Oord, Aaron van den and Dieleman, Sander and Zen, Heiga and Simonyan, Karen and Vinyals, Oriol and Graves, Alex and Kalchbrenner, Nal and Senior, Andrew and Kavukcuoglu, Koray},
  journal={arXiv preprint arXiv:1609.03499},
  year={2016}
}

@inproceedings{zhang2018end,
  title={An end-to-end deep learning architecture for graph classification},
  author={Zhang, Muhan and Cui, Zhicheng and Neumann, Marion and Chen, Yixin},
  booktitle={Thirty-Second AAAI Conference on Artificial Intelligence},
  year={2018}
}

@inproceedings{xu2019spatial,
  title={Spatial-aware graph relation network for large-scale object detection},
  author={Xu, Hang and Jiang, ChenHan and Liang, Xiaodan and Li, Zhenguo},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={9298--9307},
  year={2019}
}

@inproceedings{ying2018graph,
  title={Graph convolutional neural networks for web-scale recommender systems},
  author={Ying, Rex and He, Ruining and Chen, Kaifeng and Eksombatchai, Pong and Hamilton, William L and Leskovec, Jure},
  booktitle={Proceedings of the 24th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={974--983},
  year={2018}
}

@article{henaff2015deep,
  title={Deep convolutional networks on graph-structured data},
  author={Henaff, Mikael and Bruna, Joan and LeCun, Yann},
  journal={arXiv preprint arXiv:1506.05163},
  year={2015}
}

@article{micheli2009neural,
  title={Neural network for graphs: A contextual constructive approach},
  author={Micheli, Alessio},
  journal={IEEE Transactions on Neural Networks},
  volume={20},
  number={3},
  pages={498--511},
  year={2009},
  publisher={IEEE}
}

@article{bhattacharya2019step,
  title={Step: Spatial temporal graph convolutional networks for emotion perception from gaits},
  author={Bhattacharya, Uttaran and Mittal, Trisha and Chandra, Rohan and Randhavane, Tanmay and Bera, Aniket and Manocha, Dinesh},
  journal={arXiv preprint arXiv:1910.12906},
  year={2019}
}

@inproceedings{yan2018spatial,
  title={Spatial temporal graph convolutional networks for skeleton-based action recognition},
  author={Yan, Sijie and Xiong, Yuanjun and Lin, Dahua},
  booktitle={Thirty-second AAAI conference on artificial intelligence},
  year={2018}
}

@inproceedings{gilmer2017neural,
  title={Neural message passing for quantum chemistry},
  author={Gilmer, Justin and Schoenholz, Samuel S and Riley, Patrick F and Vinyals, Oriol and Dahl, George E},
  booktitle={Proceedings of the 34th International Conference on Machine Learning-Volume 70},
  pages={1263--1272},
  year={2017},
  organization={JMLR. org}
}

@inproceedings{atwood2016diffusion,
  title={Diffusion-convolutional neural networks},
  author={Atwood, James and Towsley, Don},
  booktitle={Advances in neural information processing systems},
  pages={1993--2001},
  year={2016}
}

@inproceedings{veli2018graph,
  title={Graph Attention Networks},
  author={Petar Veličković and Guillem Cucurull and Arantxa Casanova and Adriana Romero and Pietro Liò and Yoshua Bengio},
  booktitle={International Conference on Learning Representations},
  year={2018},
  url={https://openreview.net/forum?id=rJXMpikCZ},
}

@inproceedings{
  xu2018how,
  title={How Powerful are Graph Neural Networks?},
  author={Keyulu Xu and Weihua Hu and Jure Leskovec and Stefanie Jegelka},
  booktitle={International Conference on Learning Representations},
  year={2019},
  url={https://openreview.net/forum?id=ryGs6iA5Km},
}

@inproceedings{williams2016advanced,
  title={Advanced image classification using wavelets and convolutional neural networks},
  author={Williams, Travis and Li, Robert},
  booktitle={2016 15th IEEE international conference on machine learning and applications (ICMLA)},
  pages={233--239},
  year={2016},
  organization={IEEE}
}

@inproceedings{williams2018wavelet,
  title={Wavelet Pooling for Convolutional Neural Networks},
  author={Travis Williams and Robert Li},
  booktitle={International Conference on Learning Representations},
  year={2018},
  url={https://openreview.net/forum?id=rkhlb8lCZ},
}

@article{wang2019haarpooling,
  title={Haar graph pooling},
  author={Wang, Yu Guang and Li, Ming and Ma, Zheng and Montufar, Guido and Zhuang, Xiaosheng and Fan, Yanan},
  journal={arXiv preprint arXiv:1909.11580},
  year={2019}
}

@article{liu2019multi,
  title={Multi-level wavelet convolutional neural networks},
  author={Liu, Pengju and Zhang, Hongzhi and Lian, Wei and Zuo, Wangmeng},
  journal={IEEE Access},
  volume={7},
  pages={74973--74985},
  year={2019},
  publisher={IEEE}
}

@article{karypis1995metis,
  title={A fast and high quality multilevel scheme for partitioning irregular graphs},
  author={Karypis, George and Kumar, Vipin},
  journal={SIAM Journal on Scientific Computing},
  volume={20},
  number={1},
  pages={359--392},
  year={1998},
  publisher={SIAM}
}

@article{dhillon2007weighted,
  title={Weighted graph cuts without eigenvectors a multilevel approach},
  author={Dhillon, Inderjit S and Guan, Yuqiang and Kulis, Brian},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={29},
  number={11},
  pages={1944--1957},
  year={2007},
  publisher={IEEE}
}

@article{hammond2011wavelets,
  title={Wavelets on graphs via spectral graph theory},
  author={Hammond, David K and Vandergheynst, Pierre and Gribonval, R{\'e}mi},
  journal={Applied and Computational Harmonic Analysis},
  volume={30},
  number={2},
  pages={129--150},
  year={2011},
  publisher={Elsevier}
}

@article{chui2015representation,
  title={Representation of functions on big data: graphs and trees},
  author={Chui, CK and Filbir, F and Mhaskar, HN},
  journal={Applied and Computational Harmonic Analysis},
  volume={38},
  number={3},
  pages={489--509},
  year={2015},
  publisher={Elsevier}
}

@article{gavish2012sampling,
  title={Sampling, denoising and compression of matrices by coherent matrix organization},
  author={Gavish, Matan and Coifman, Ronald R},
  journal={Applied and Computational Harmonic Analysis},
  volume={33},
  number={3},
  pages={354--369},
  year={2012},
  publisher={Academic Press}
}

@inproceedings{ying2018hierarchical,
  title={Hierarchical graph representation learning with differentiable pooling},
  author={Ying, Zhitao and You, Jiaxuan and Morris, Christopher and Ren, Xiang and Hamilton, Will and Leskovec, Jure},
  booktitle={Advances in neural information processing systems},
  pages={4800--4810},
  year={2018}
}

@article{cangea2018towards,
  title={Towards sparse hierarchical graph classifiers},
  author={Cangea, C{\u{a}}t{\u{a}}lina and Veli{\v{c}}kovi{\'c}, Petar and Jovanovi{\'c}, Nikola and Kipf, Thomas and Li{\`o}, Pietro},
  journal={arXiv preprint arXiv:1811.01287},
  year={2018}
}

@inproceedings{gao2019graph,
  title={Graph U-nets},
  author={Gao, Hongyang and Ji, Shuiwang},
  booktitle={the 36th International Conference on Machine Learning (ICML)},
  year={2019}
}

@inproceedings{knyazev2019understanding,
  title={Understanding Attention and Generalization in Graph Neural Networks},
  author={Knyazev, Boris and Taylor, Graham W and Amer, Mohamed},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4204--4214},
  year={2019}
}

@inproceedings{ma2019graph,
  title={Graph convolutional networks with eigenpooling},
  author={Ma, Yao and Wang, Suhang and Aggarwal, Charu C and Tang, Jiliang},
  booktitle={Proceedings of the 25th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={723--731},
  year={2019}
}

@article{hoang2019revisiting,
  title={Revisiting graph neural networks: All we have is low-pass filters},
  author={Hoang, NT and Maehara, Takanori},
  journal={arXiv preprint arXiv:1905.09550},
  year={2019}
}

@article{xu2018powerful,
  title={How powerful are graph neural networks?},
  author={Xu, Keyulu and Hu, Weihua and Leskovec, Jure and Jegelka, Stefanie},
  journal={arXiv preprint arXiv:1810.00826},
  year={2018}
}

@article{wu2020comprehensive,
  title={A comprehensive survey on graph neural networks},
  author={Wu, Zonghan and Pan, Shirui and Chen, Fengwen and Long, Guodong and Zhang, Chengqi and Philip, S Yu},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  year={2020, DOI: 10.1109/TNNLS.2020.2978386},
  publisher={IEEE}
}

@INPROCEEDINGS{Morris2017Glocalized,
  author={C. {Morris} and K. {Kersting} and P. {Mutzel}},
  booktitle={2017 IEEE International Conference on Data Mining (ICDM)},
  title={Glocalized Weisfeiler-Lehman Graph Kernels: Global-Local Feature Maps of Graphs},
  year={2017},
  pages={327-336}
}

@article{von2007tutorial,
  title={A tutorial on spectral clustering},
  author={Von Luxburg, Ulrike},
  journal={Statistics and computing},
  volume={17},
  number={4},
  pages={395--416},
  year={2007},
  publisher={Springer}
}

@inproceedings{hamilton2017inductive,
  title={Inductive representation learning on large graphs},
  author={Hamilton, Will and Ying, Zhitao and Leskovec, Jure},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1024--1034},
  year={2017}
}

@inproceedings{monti2017geometric,
  title={Geometric deep learning on graphs and manifolds using mixture model cnns},
  author={Monti, Federico and Boscaini, Davide and Masci, Jonathan and Rodola, Emanuele and Svoboda, Jan and Bronstein, Michael M},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={5115--5124},
  year={2017}
}

@inproceedings{kondor2016multiscale,
  title={The multiscale laplacian graph kernel},
  author={Kondor, Risi and Pan, Horace},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2990--2998},
  year={2016}
}

@article{kriege2020survey,
  title={A survey on graph kernels},
  author={Kriege, Nils M and Johansson, Fredrik D and Morris, Christopher},
  journal={Applied Network Science},
  volume={5},
  number={1},
  pages={1--42},
  year={2020},
  publisher={Springer}
}

@article{lee2019self,
  title={Self-attention graph pooling},
  author={Lee, Junhyun and Lee, Inyeop and Kang, Jaewoo},
  journal={arXiv preprint arXiv:1904.08082},
  year={2019}
}

@inproceedings{duvenaud2015convolutional,
  title={Convolutional networks on graphs for learning molecular fingerprints},
  author={Duvenaud, David K and Maclaurin, Dougal and Iparraguirre, Jorge and Bombarell, Rafael and Hirzel, Timothy and Aspuru-Guzik, Al{\'a}n and Adams, Ryan P},
  booktitle={Advances in neural information processing systems},
  pages={2224--2232},
  year={2015}
}

@article{noutahi2019towards,
  title={Towards interpretable sparse graph representation learning with laplacian pooling},
  author={Noutahi, Emmanuel and Beani, Dominique and Horwood, Julien and Tossou, Prudencio},
  journal={arXiv preprint arXiv:1905.11577},
  year={2019}
}

@article{vijay2020benchmarking,
  title={Benchmarking Graph Neural Networks},
  author={Vijay, Prakash, Dwivedi and Chaitanya, K. Joshi and Thomas, Laurent and Yoshua, Bengio and Xavier, Bresson},
  journal={arXiv preprint arXiv:2003.00982v1},
  year={2020}
}

@article{zhou2018graph,
  title={Graph neural networks: A review of methods and applications},
  author={Zhou, Jie and Cui, Ganqu and Zhang, Zhengyan and Yang, Cheng and Liu, Zhiyuan and Wang, Lifeng and Li, Changcheng and Sun, Maosong},
  journal={arXiv preprint arXiv:1812.08434},
  year={2018}
}

@article{scarselli2008graph,
  title={The graph neural network model},
  author={Scarselli, Franco and Gori, Marco and Tsoi, Ah Chung and Hagenbuchner, Markus and Monfardini, Gabriele},
  journal={IEEE Transactions on Neural Networks},
  volume={20},
  number={1},
  pages={61--80},
  year={2008},
  publisher={IEEE}
}

@inproceedings{gori2005new,
  title={A new model for learning in graph domains},
  author={Gori, Marco and Monfardini, Gabriele and Scarselli, Franco},
  booktitle={Proceedings of the IEEE International Joint Conference on Neural Networks},
  volume={2},
  pages={729--734},
  year={2005},
  organization={IEEE}
}

@article{scarselli2008computational,
  title={Computational capabilities of graph neural networks},
  author={Scarselli, Franco and Gori, Marco and Tsoi, Ah Chung and Hagenbuchner, Markus and Monfardini, Gabriele},
  journal={IEEE Transactions on Neural Networks},
  volume={20},
  number={1},
  pages={81--102},
  year={2008},
  publisher={IEEE}
}

@book{chung1997spectral,
  title={Spectral graph theory},
  author={Chung, Fan RK and Graham, Fan Chung},
  number={92},
  year={1997},
  publisher={American Mathematical Society}
}

